Looking Back: Field theory of transiently chiral active particles

We derive a Doi-Peliti Field Theory for transiently chiral active particles in two dimensions, that is, active Brownian particles that undergo tumbles via a diffusing reorientation angle. Using this framework, we compute the mean squared displacement for both uniformly distributed and fixed initial reorientations. We also calculate an array of orientation-based observables, to quantify the transiently chiral behaviour observed.

==> selected_gp_macros.tex <==
\newcommand{\plaind}{\mathrm{d}}
\newcommand{\dint}[1]{\mathchoice{\!\plaind#1\,}{\!\plaind#1\,}{\!\plaind#1\,}{\!\plaind#1\,}}
\newcommand{\ddint}[1]{\ddintx{#1}{d}}
\newcommand{\dnint}[1]{\ddintx{#1}{n}}
\newcommand{\ddintx}[2]{\mathchoice{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}}
\newcommand{\ddMOneint}[1]{\mathchoice{\!\plaind^{d-1}#1\,}{\!\plaind^{d-1}#1\,}{\!\plaind^{d-1}#1\,}{\!\plaind^{d-1}#1\,}}
\newcommand{\Xddint}[2]{\mathchoice{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}}
\newcommand{\dbar}{\text{\dj}}
\newcommand{\deltabar}{\delta\mkern-6mu\mathchar'26}
\newcommand{\dintbar}[1]{\mathchoice{\!\dbar#1\,}{\!\dbar#1\,}{\!\dbar#1\,}{\!\dbar#1\,}}
\newcommand{\ddintbar}[1]{\mathchoice{\!\dbar^d#1\,}{\!\dbar^d#1\,}{\!\dbar^d#1\,}{\!\dbar^d#1\,}}
\newcommand{\ddMOneintbar}[1]{\mathchoice{\!\dbar^{d-1}#1\,}{\!\dbar^{d-1}#1\,}{\!\dbar^{d-1}#1\,}{\!\dbar^{d-1}#1\,}}
\newcommand{\Dint}[1]{\mathcal{D}\!#1\,}
\DeclareFontFamily{U}{wncy}{}
\DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
\DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
\DeclareMathSymbol{\sha}{\mathord}{mcy}{"58}


\newcommand{\MCLineVsMathEnv}[2]{\mathchoice{#1}{#2}{#2}{#2}}
\newcommand{\dX}[1]{\plaind #1}
\newcommand{\dx}{\dX{x}}
\newcommand{\ds}{\dX{s}}
\newcommand{\dt}{\dX{t}}
\newcommand{\ddX}[1]{\MCLineVsMathEnv{\frac{\plaind}{\plaind #1}}{\plaind/\plaind #1}}
\newcommand{\ddt}{\ddX{t}}
\newcommand{\ddx}{\ddX{x}}
\newcommand{\dds}{\ddX{s}}
\newcommand{\ddXX}[2]{\MCLineVsMathEnv{\frac{\plaind #1}{\plaind #2}}{\plaind #1/\plaind #2}}
\newcommand{\ddtX}[1]{\ddXX{#1}{t}}
\newcommand{\ddxX}[1]{\ddXX{#1}{x}}
\newcommand{\ddsX}[1]{\ddXX{#1}{s}}
\newcommand{\ppX}[1]{\MCLineVsMathEnv{\frac{\partial}{\partial #1}}{\partial/\partial #1}}
\newcommand{\ppx}{\ppX{x}}
\newcommand{\ppt}{\ppX{t}}
\newcommand{\ppXX}[2]{\MCLineVsMathEnv{\frac{\partial #1}{\partial #2}}{\partial #1/\partial #2}}
\newcommand{\pptX}[1]{\ppXX{#1}{t}}
\newcommand{\ppxX}[1]{\ppXX{#1}{x}}
\newcommand{\ppsX}[1]{\ppXX{#1}{s}}

\usepackage{dsfont}
\newcommand{\OLDgpset}[1]{\mathbb{#1}}
\newcommand{\gpset}[1]{\mathds{#1}}

\newcommand{\canetset}[1]{{\mathchoice {\hbox{$\sf\textstyle #1\kern-0.4em #1$}}
{\hbox{$\sf\textstyle #1\kern-0.4em #1$}}
{\hbox{$\sf\scriptstyle #1\kern-0.3em #1$}}
{\hbox{$\sf\scriptscriptstyle #1\kern-0.2em #1$}}}}

\newcommand{\Nset}{\gpset{N}}
\newcommand{\Zset}{\gpset{Z}}
\newcommand{\Qset}{\gpset{Q}}
\newcommand{\Rset}{\gpset{R}}
\newcommand{\Cset}{\gpset{C}}
\newcommand{\Sset}{\gpset{S}}
\newcommand{\Wset}{\gpset{W}}


\DeclareMathOperator*{\SumInt}{%
\mathchoice%
  {\ooalign{$\displaystyle\sum$\cr\hidewidth$\displaystyle\int$\hidewidth\cr}}
  {\ooalign{\raisebox{.14\height}{\scalebox{.7}{$\textstyle\sum$}}\cr\hidewidth$\textstyle\int$\hidewidth\cr}}
  {\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
  {\ooalign{\raisebox{.2\height}{\scalebox{.6}{$\scriptstyle\sum$}}\cr$\scriptstyle\int$\cr}}
}



\def\nbZ{{\mathchoice {\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\scriptstyle Z\kern-0.3em Z$}}
{\hbox{$\sf\scriptscriptstyle Z\kern-0.2em Z$}}}}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}


\newcommand{\gpvec}[1]{\mathbf{#1}}

\newcommand{\zerovec}{\gpvec{0}}
\newcommand{\nullvec}{\zerovec}
\newcommand{\avec}{\gpvec{a}}
\newcommand{\bvec}{\gpvec{b}}
\newcommand{\cvec}{\gpvec{c}}
\newcommand{\dvec}{\gpvec{d}}
\newcommand{\evec}{\gpvec{e}}
\newcommand{\fvec}{\gpvec{f}}
\newcommand{\gvec}{\gpvec{g}}
\newcommand{\ivec}{\gpvec{i}}
\newcommand{\jvec}{\gpvec{j}}
\newcommand{\kvec}{\gpvec{k}}
\newcommand{\ellvec}{\gpvec{\ell}}
\newcommand{\mvec}{\gpvec{m}}
\newcommand{\nvec}{\gpvec{n}}
\newcommand{\pvec}{\gpvec{p}}
\newcommand{\qvec}{\gpvec{q}}
\newcommand{\rvec}{\gpvec{r}}
\newcommand{\svec}{\gpvec{s}}
\newcommand{\uvec}{\gpvec{u}}
\newcommand{\vvec}{\gpvec{v}}
\newcommand{\wvec}{\gpvec{w}}
\newcommand{\xvec}{\gpvec{x}}
\newcommand{\yvec}{\gpvec{y}}
\newcommand{\zvec}{\gpvec{z}}

\newcommand{\Avec}{\gpvec{A}}
\newcommand{\Bvec}{\gpvec{B}}
\newcommand{\Cvec}{\gpvec{C}}
\newcommand{\Evec}{\gpvec{E}}
\newcommand{\Fvec}{\gpvec{F}}
\newcommand{\Hvec}{\gpvec{H}}
\newcommand{\Ivec}{\gpvec{I}}
\newcommand{\Jvec}{\gpvec{J}}
\newcommand{\Kvec}{\gpvec{K}}
\newcommand{\Mvec}{\gpvec{M}}
\newcommand{\Nvec}{\gpvec{N}}
\newcommand{\Pvec}{\gpvec{P}}
\newcommand{\Qvec}{\gpvec{Q}}
\newcommand{\Rvec}{\gpvec{R}}
\newcommand{\Svec}{\gpvec{S}}
\newcommand{\Uvec}{\gpvec{U}}
\newcommand{\Vvec}{\gpvec{V}}
\newcommand{\Wvec}{\gpvec{W}}
\newcommand{\Xvec}{\gpvec{X}}
\newcommand{\Yvec}{\gpvec{Y}}
\newcommand{\Zvec}{\gpvec{Z}}

% $\boldsymbol{\alpha}$ vs $\bm{\alpha}$ vs $\mathbf{w}$ vs w vs $\boldsymbol{w}$
\newcommand{\alphavec}{\bm{\alpha}}
\newcommand{\betavec}{\bm{\beta}}
\newcommand{\deltavec}{\bm{\delta}}
\newcommand{\etavec}{\bm{\eta}}
\newcommand{\gammavec}{\bm{\gamma}}
\newcommand{\epsilonvec}{\bm{\epsilon}}
\newcommand{\muvec}{\bm{\mu}}
\newcommand{\nuvec}{\bm{\nu}}
\newcommand{\phivec}{\bm{\phi}}
\newcommand{\varphivec}{\bm{\varphi}}
%\newcommand{\Phivec}{\bm{\Phi}}
\newcommand{\xivec}{\bm{\xi}}
\newcommand{\zetavec}{\bm{\zeta}}


\newcommand{\transpose}{\mathsf{T}}
\renewcommand{\det}[1]{\mathchoice
{\operatorname{det}\left(#1\right)}
{\operatorname{det}(#1)}
{\operatorname{det}(#1)}
{\operatorname{det}(#1)}
}
\newcommand{\ident}{\mathbf{1}}
\newcommand{\unity}{\ident}
%\newcommand{\Trace}{\operatorname{Tr}}

\newcommand*\laplace{\mathop{}\!\mathbin\bigtriangleup}


%\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}

\renewcommand{\AC}{\mathcal{A}}
\newcommand{\BC}{\mathcal{B}}
\newcommand{\DC}{\mathcal{D}}
\newcommand{\EC}{\mathcal{E}}
\newcommand{\FC}{\mathcal{F}}
\newcommand{\GC}{\mathcal{G}}
\newcommand{\HC}{\mathcal{H}}
\newcommand{\IC}{\mathcal{I}}
\newcommand{\JC}{\mathcal{J}}
\newcommand{\KC}{\mathcal{K}}
\newcommand{\LC}{\mathcal{L}}
\newcommand{\MC}{\mathcal{M}}
%\newcommand{\NC}{\mathcal{N}}
\newcommand{\OC}{\mathcal{O}}
\newcommand{\PC}{\mathcal{P}}
\newcommand{\VC}{\mathcal{V}}
\newcommand{\WC}{\mathcal{W}}
\newcommand{\XC}{\mathcal{X}}
\newcommand{\ZC}{\mathcal{Z}}


\newcommand{\Gtilde}{\tilde{G}}
\newcommand{\GCtilde}{\tilde{\GC}}
\newcommand{\jtilde}{\tilde{j}}
\newcommand{\mtilde}{\tilde{m}}
\newcommand{\stilde}{\tilde{s}}
\newcommand{\ttilde}{\tilde{t}}
\newcommand{\utilde}{\tilde{u}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Gammatilde}{\tilde{\Gamma}}
\newcommand{\gammatilde}{\tilde{\gamma}}
\newcommand{\phitilde}{\tilde{\phi}}
\newcommand{\adagger}{a^{\dagger}}
\newcommand{\chidagger}{\chi^{\dagger}}
\newcommand{\phidagger}{\phi^{\dagger}}
\newcommand{\psitilde}{\tilde{\psi}}
\newcommand{\tautilde}{\tilde{\tau}}
\newcommand{\chitilde}{\tilde{\tau}}


\newcommand{\Ghat}{\hat{G}}
\newcommand{\What}{\hat{W}}
\newcommand{\Gammahat}{\hat{\Gamma}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\jhat}{\hat{j}}

\newcommand{\half}{\mathchoice{\frac{1}{2}}{(1/2)}{\frac{1}{2}}{(1/2)}}
\newcommand{\threehalf}{\mathchoice{\frac{3}{2}}{(3/2)}{\frac{3}{2}}{(3/2)}}
\newcommand{\fourth}{\mathchoice{\frac{1}{4}}{(1/4)}{\frac{1}{4}}{(1/4)}}
\newcommand{\third}{\mathchoice{\frac{1}{3}}{(1/3)}{\frac{1}{3}}{(1/3)}}
\newcommand{\quarter}{\fourth}

\newcommand{\EXP}[1]{\operatorname{exp}\!\Bigg\{#1\Bigg\}}
\newcommand{\Exp}[1]{\operatorname{exp}\left(#1\right)}
\renewcommand{\exp}[1]{\mathchoice%
{\mathrm{e}^{#1}}%
{\operatorname{exp}(#1)}
{\operatorname{exp}\left(#1\right)}%
{\operatorname{exp}\left(#1\right)}}

\newcommand{\sgn}{\operatorname{sgn}}


\newcommand{\elabel}[1]{\label{eq:#1}}
%\newcommand{\eref}[1]{(\ref{eq:#1})}
%\newcommand{\Eref}[1]{\mbox{Eq.~(\ref{eq:#1})}}
\newcommand{\Erefs}[1]{\mbox{Eqs.~(\ref{eq:#1})}}

\newcommand{\seclabel}[1]{\label{sec:#1}}
%\newcommand{\sref}[1]{\ref{sec:#1}}
%\newcommand{\Sref}[1]{Section~\ref{sec:#1}}
\newcommand{\Srefs}[1]{Sections~\ref{sec:#1}}
\newcommand{\ASref}[1]{Appendix~\ref{sec:#1}}

\newcommand{\flabel}[1]{\label{fig:#1}}
%\newcommand{\fref}[1]{Fig.~\ref{fig:#1}}
%\newcommand{\Fref}[1]{Figure~\ref{fig:#1}}
\newcommand{\subfref}[1]{\subref{fig:#1}}

\newcommand{\tlabel}[1]{\label{tab:#1}}
\newcommand{\Tref}[1]{Tab.~\ref{tab:#1}}
%\newcommand{\tref}[1]{tab.~\ref{tab:#1}}

\newcommand{\latin}[1]{{\it #1}}
\newcommand{\ie}{\latin{i.e.}\@\xspace}
\newcommand{\eg}{\latin{e.g.}\@\xspace}
\newcommand{\cf}{\latin{cf.}\@\xspace}
\newcommand{\etc}{\latin{etc.}\@\xspace}
\newcommand{\viz}{\latin{viz.}\@\xspace}
%\newcommand{\etal}{\latin{et~al}.\@\xspace}
\newcommand{\vs}{\latin{vs}.\@\xspace}
\newcommand{\glossarykeyword}[1]{\textcolor{blue}{\bf #1}}
\newcommand{\keyword}[1]{{\bf #1}}
\newcommand{\pname}[1]{\textsc{#1}} 
\newcommand{\eetin}[1]{\emph{#1}}
\newlength \standardfigwidth
\setlength \standardfigwidth{0.66\linewidth}


\DeclareMathAlphabet{\matheub}{U}{eur}{m}{n}
\newcommand{\unitX}[1]{\matheub{#1}}
\newcommand{\Angstrom}{\unitX{\AA}}
\newcommand{\dimof}[1]{\left[#1\right]}
\newcommand{\unitL}{\unitX{L}}
\newcommand{\unitT}{\unitX{T}}
\newcommand{\unitA}{\unitX{A}}
\newcommand{\unitB}{\unitX{B}}
\newcommand{\unitz}{\unitX{z}}



\newcommand{\Adim}{\mathtt{A}}
\newcommand{\Bdim}{\mathtt{B}}
\newcommand{\Cdim}{\mathtt{C}}
\newcommand{\Ldim}{\mathtt{L}}


\newcommand{\V}[1]{\text{Var}\left(#1\right)}
\newcommand{\E}[1]{\text{E}\left[#1\right]}

\newcommand{\renorm}{\mathcal{R}}
\newcommand{\ai}[4]{{\left[\begin{smallmatrix}\textcolor{cyan}{#1}&\textcolor{cyan}{#2}\\\textcolor{orange}{#3}&\textcolor{orange}{#4}\end{smallmatrix}\right]}}
\newcommand{\Gammaai}[4]{\Gamma^{\ai{#1}{#2}{#3}{#4}}}
\newcommand{\Gai}[4]{G^{\ai{#1}{#2}{#3}{#4}}}
\newcommand{\xPs}{P_{\text{surv}}}
\newcommand{\Ps}{P_{\text{s}}}


\DeclareMathOperator{\diag}{diag}


%\usepackage{tikz}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{arrows,shapes,decorations,automata,backgrounds,petri}
\usetikzlibrary{calc}
\usetikzlibrary{patterns}
\usetikzlibrary{decorations.text}


\newcommand{\spave}[1]{\overline{#1}}
\newcommand{\ave}[2][]{\mathchoice%
{\left\langle #2 \right\rangle_{#1}}%
{\langle #2\rangle_{#1}}
{\langle #2\rangle_{#1}}%
{\langle #2\rangle_{#1}}}



\newcommand{\Psurv}{P_\text{s}}
\newcommand{\cov}[2]{\text{Cov}\left(#1,#2\right)}
\newcommand{\Pext}{P_\text{e}(t)}
%\newcommand{\var}[1]{\text{Var}\left( #1 \right)}
\newcommand{\pgf}{f}
\newcommand{\union}{\cup}
\newcommand{\plaint}{\mathrm{t}}
%\newcommand{\bra}[1]{\left\langle#1\right|}
%\newcommand{\ket}[1]{\left|#1\right\rangle}
%\newcommand{\braket}[2]{\left\langle#1\middle|#2\right\rangle}
\newcommand{\sandwich}[3]{\left\langle#1\middle|#2\middle|#3\right\rangle}
\newcommand{\creat}{a^\dagger}
\makeatletter
\newcommand{\creatX}[2][]{a^{\@ifempty{#1}{\dagger}{\dagger\,#1}}\@ifempty{#2}{}{(#2)}}
\makeatother
\newcommand{\creatDS}{\tilde{a}}
\makeatletter
\newcommand{\creatDSX}[2][]{\@ifempty{#1}{\creatDS}{\creatDS^{#1}}\@ifempty{#2}{}{(#2)}}
\makeatother
\newcommand{\annih}{a}
\makeatletter
\newcommand{\annihX}[2][]{a\@ifempty{#1}{}{^{#1}}\@ifempty{#2}{}{(#2)}}
\newcommand{\kernel}[1]{K\@ifempty{#1}{}{\,\!\!\left(#1\right)}}
\newcommand{\kernelDeri}[1]{K'\@ifempty{#1}{}{\left(#1\right)}}
\newcommand{\Kbar}{\overline{K}}
\newcommand{\Kmatrix}{\mathsf{K}}
\newcommand{\Okernel}[1]{K\left(#1\right)}
\newcommand{\OkernelDeri}[1]{K'\left(#1\right)}


